README: Bridging Medical Jargon and Lay Understanding for Patient Education through Data-Centric NLP

The advancement in healthcare has shifted focus toward patient-centric approaches, particularly in self-care and patient education, facilitated by access to Electronic Health Records (EHR). However, medical jargon in EHRs poses significant challenges in patient comprehension. To address this, we introduce a new task of automatically generating lay definitions, aiming to simplify complex medical terms into patient-friendly lay language. We first created the README dataset, an extensive collection of over 50,000 unique (medical term, lay definition) pairs and 300,000 mentions, each offering context-aware lay definitions manually annotated by domain experts. We have also engineered a data-centric Human-AI pipeline that synergizes data filtering, augmentation, and selection to improve data quality. We then used README as the training data for models and leveraged a Retrieval-Augmented Generation method to reduce hallucinations and improve the quality of model outputs. Our extensive automatic and human evaluations demonstrate that open-source mobile-friendly models, when fine-tuned with high-quality data, are capable of matching or even surpassing the performance of state-of-the-art closed-source large language models like ChatGPT. This research represents a significant stride in closing the knowledge gap in patient education and advancing patient-centric healthcare solutions.

==> sub_tex_files/EAE.tex <==
\subsubsection{Examiner (expert-annotated data)}
Initially, basic data cleaning, as outlined in Section \ref{Sec:data_construction}, was applied. To enhance this, we employed GPT-3.5-turbo, using a few-shot learning approach with seven examples - four demonstrating acceptable data points and three showing unacceptable ones. 
These prompts served as the `Human' element in our Human-AI-in-the-loop model, as depicted in Figure \ref{fig:human-ai-loop} and detailed in Algorithm~\ref{algo:data_cleaning}. The prompts are detailed in Table 5. We choose GPT-3.5-turbo here because recent work~\cite{remy2023automatic} and our evaluation (\ref{method:soft_hard_correlation} and \ref{Sec:results}) show that the definitions it generates for medical terms can reach a human-satisfying level.
Post-cleaning, approximately 40\% of UMLS general definitions were deemed suitable for model training. The suitable data points were archived in README-v2, while the unsuitable ones were stored in README-v3.
To minimize computing costs, we excluded EHRs and took all the unique data points. This was done because, in many cases, we have the same jargon term, general definition from UMLS, and lay definition but different EHR's. 
This reduced our dataset from 308,239 to 51,623 data points. Upon processing these through GPT-3.5-turbo, 11,765 were classified as `good' quality general definitions, and 39,856 as `bad'. A subsequent SQL join with contextual data removed earlier resulted in 113,659 `good' and 194,580 `bad' general definitions. After eliminating duplicates, the final count for bad general definitions in README-v3 was 177,140.

\vspace{-3mm} % Reduce space before the algorithm
\begin{algorithm}
  \caption{Algorithm for Data Cleaning}
  \label{algo:data_cleaning}
  \SetKwInOut{Input}{inputs}
  \SetKwInOut{Output}{output}
  \SetKwProg{READMEEAE}{README-EAE}{}{}

  \READMEEAE{}{
    \Input{README-v1}
    \Output{Final README-v6 dataset with best general definitions and lay definitions}
    $Initialize:$
    $exam_{p} = examiner prompt for gpt3$\;
    $aug_{p} = augmenter prompts for ChatGPT$\;
    \ForEach{$datapoint : README - v1$}{%
     \If{$exam_{p}(datapoint) == yes$}{
     README-v2.add(datapoint)\;
     }
     \Else{
     README-v3.add(datapoint);
     }
    }
    \ForEach{$datapoint : README - v3$}{%
     $temp = aug_{p}(datapoint)$\;
     README-v4.add(temp)\;
     \If{$exam_{p}(temp) == yes$}{
     README-v5.add(temp)\;
     }
     \Else{
     README-v6.add(temp)\;
     }
    }
    \KwRet{README-v6}\;
  }
\end{algorithm}
\vspace{-7mm} % Reduce space before the 

\subsubsection{Augmenter}
Given the low yield of usable UMLS definitions, we employed ChatGPT, a recent LLM by OpenAI, to augment our dataset. The augmentation process, a critical part of our Data-centric pipeline, involved the system prompt: "Generate a general definition of the term for a professional medical student." Accompanied by two examples(Table 5), this step aimed to create complex yet general definitions suitable for professional medical students. The outcome of this process was README-v4, containing 171,831 newly generated definitions.


\subsubsection{Examiner (AI-synthetic data)}
The ChatGPT-generated definitions underwent a second cleaning round using the same methodology as in Examiner (expert-annotated data). Here, approximately 56\% of the ChatGPT definitions were found suitable for model training, with the remaining being either contextually inappropriate or incompatible with the expert-provided lay definitions. The final tally was 96,585 `good' and 75,068 `bad' general definitions, stored in README-v5 and README-v6, respectively.



\subsubsection{Data Quality}
\label{method:soft_hard_correlation}
The final stage involved preparing the training data, which comprised good definitions from README-v2 and README-v5. This data was split into three categories: human examination data (also be used as final test data since medical experts examine this split), out-of-distribution (OOD) evaluation data, and training data, where we make sure the medical jargon in human examination and OOD evaluation will not appear in the training split. The human examination split consisted of 1000 unique terms, each accompanied by general definitions to be rated based on two criteria:


\begin{enumerate}
[topsep=0.5pt,itemsep=0.2ex,partopsep=0.2ex,parsep=.20ex]
    \item Hard Correlation: Marked `Yes' if the lay definition closely rephrases or shares significant wording with the general definition, implying comprehensibility without advanced medical knowledge.
    \item Soft Correlation: Marked `Yes' if the general definition accurately represents the term but is slightly contextually misaligned; marked `No' if the definition is incorrect or overly verbose, complicating the derivation of a lay definition.
\end{enumerate}

Here is one example for \textbf{Term} `von Willebrand disease':

\textbf{Expert Definition(lay definition)}: A bleeding disorder. It affects the blood's ability to clot

\textbf{General definition}: Hereditary or acquired coagulation disorder characterized by a qualitative or quantitative deficiency of the von Willebrand factor. The latter plays an important role in platelet adhesion. Signs and symptoms include bruises, nose bleeding, gum bleeding following a dental procedure, heavy menstrual bleeding, and gastrointestinal bleeding.

Although the lay definition is not incorrect, it is very wordy and complex and matches less to the lay definition. We consider this soft correlated and not hard correlated.

A Hard Correlation automatically implies a Soft Correlation. Our findings revealed that 88\% of README-v2 and 100\% of README-v5 met the Hard Correlation criteria. There is a 100\% soft Correlation criteria for both README-v2 and README-v5. 

==> sub_tex_files/EAE_prompts.tex <==
% \twocolumn
% \subsection{Prompts}\label{prompts}
\lstset{
    basicstyle=\ttfamily,
    columns=fullflexible,
    breaklines=true,
    postbreak=\mbox{\textcolor{red}{$\hookrightarrow$}\space}
}
{\tiny
% \begin{table}%[ht]
% \caption{}
% \label{prompts}
\centering
\begin{tabular}{|p{7.6cm}|}
\hline
\textbf{Prompt} \\ \hline
\begin{lstlisting}
Examiner - 1

model = "gpt-3.5-turbo(ChatGPT API)"
[This examiner prompt does not use context as discussed in section 3.2.1]

Decide whether the general definition is correct.

If we can generate the lay definition from the general definition then answer is yes.

term : mg
general definition : this is short for milligram which is 1/1000 of a gram usually considered a small amount.
lay definition : A tiny amount of something, usually a drug.
answer : yes

term : vitamin c
general definition : [`A nutrient that the body needs in small amounts to function and stay healthy. Vitamin C helps fight infections, heal wounds, and keep tissues healthy. It is an antioxidant that helps prevent cell damage caused by free radicals (highly reactive chemicals). Vitamin C is found in all fruits and vegetables, especially citrus fruits, strawberries, cantaloupe, green peppers, tomatoes, broccoli, leafy greens, and potatoes. It is water-soluble (can dissolve in water) and must be taken in every day. Vitamin C is being studied in the prevention and treatment of some types of cancer.']
lay definition : A nutrient needed by the body to form and maintain bones, blood vessels, and skin.
answer : yes

term : nodule
general definition : [`A small lump, swelling or collection of tissue.']
lay definition : A growth or lump that may be cancerous or not.
answer : yes

term : qd
general definition : [`Occurring or done each day.']
lay definition : Every day.
answer : yes

If the general definition contains many words from the term then answer is no.

term : prochlorperzine 
general definition : [`prochlorperzine', ` ']
lay definition : A drug used to prevent or reduce nausea and vomiting.
answer : no

term : mg
general definition : [`mg']
lay definition : A tiny amount of something, usually a drug.
answer : no

If the lay definition can not be generated by the general definition then answer is no.

term : Virt - Vite
general definition : [`Virt', ` - ', `The determination of the amount of Vitamin E present in a sample.']
lay definition : A mix of vitamins. It provides vitamin B-6, vitamin B-12 and folic acid to people who do not have enough of these for good health.
answer : no
\end{lstlisting}
\\ \hline
 
\begin{lstlisting}
Augmenter

system_prompt = "your job is to generate a general definition of the term for a professional medical student"
model="gpt-3.5-turbo(ChatGPT API)",
messages=[
        {"role": "system", "content": system_prompt},
        {"role": "user", "content": ""},
        {"role": "user", "content": "term : incisional."},
        {"role": "assistant", "content": "general definition : An intentional cut made to an individual's body with the intent of performing a diagnostic or therapeutic intervention."},
        {"role": "user", "content": "term : PO"},
        {"role": "assistant", "content": "general definition : Of, or relating to, or affecting, or for use in the mouth.."},
        {"role": "user", "content": prompt_t}
    ]
\end{lstlisting}
\\ \hline


\begin{lstlisting}
Examiner - 2

model = "gpt-3.5-turbo(ChatGPT API)"
exactly same as that of Examiner - 1
\end{lstlisting}
\\ \hline
% $p\delta$  & 
% \begin{lstlisting}
% In this task, you need to provide suggestions to modify the instruction in our SOAP notes writing system, which uses a model to generate SOAP notes from the doctor-patient conversation according to manually created instructions.
% Specifically, we feed the AI a conversation snippet and the target section in the SOAP note and ask it to generate the corresponding summary.
% But we found that the instruction in the current system is not perfect, so we need you to modify the instruction for this model to improve our system.

% The instruction now in our system:
% [Intial generic prompt or prompt iterations]
% Suggestions from summary [i]:
% [suggestions]
% Here are some of the requirements you need to be aware of when modifying the instruction in our system:
% 1) For better generalization, what you suggest should be abstracted as high-level criteria as much as possible instead of only describing the details
% 2) We will improve the instructions based on your suggestions. If I re-provide the system with the conversation snippet and the target section in the SOAP note, it needs to be able to generate the reference summary using your new suggested instructions.
% 3) The instruction now in our system is for the zero-shot setting, don't try to add any examples to the instruction.
% 4) We are currently only focusing on this target section, so you don't need to consider the situation of other sections in the SOAP note, just optimize the instructions completely for this section.

% Let's think step by step. First, briefly summarize the suggestions of all the data to get a final suggestion containing only the highest priority requirement, then output your modified instruction for our system based on the final suggestion.
% Return the output as a dictionary object, adhering to the following structure:
% {"final suggestion": ..., "new instruction": ...}
% Please provide your response solely in the dictionary format without including any additional text.
% \end{lstlisting}
% \\ \hline

\end{tabular}
% \end{table}
}
% \begin{center}
\small
Table 5: All Examiner-Augmenter-Examine prompts.


% \twocolumn

==> sub_tex_files/auto_evaluation.tex <==
% \paragraph{ROUGE, METEOR and UMLS-F1}
Models are evaluated with full-length F1-scores of ROUGE~\cite{lin2004rouge} and METEOR~\cite{banarjee2005}. We use QuickUMLS\footnote{https://github.com/Georgetown-IR-Lab/QuickUMLS} to extract medical concepts from both model-generated and ground truth lay definitions and then calculate F1-scores for these two lists of concepts, which is named UMLS-F1~\cite{adams2023meta}.


==> sub_tex_files/conclusion.tex <==
In conclusion, our study underscores the potential of NLP to democratize medical knowledge, enabling patient-centric care by simplifying complex medical terminology. 
By crafting the README dataset and integrating a data-centric Human-AI collaboration, we have not only enriched the dataset quality but also broadened the horizons for training AI models in resource-constrained scenarios. 
Our findings reveal that even smaller, open-source models can rival the capabilities of advanced, proprietary systems like ChatGPT when fine-tuned with meticulously curated data. 
This research paves the way for innovative patient education tools, making strides toward a future where all patients can navigate their health information with ease and understanding.

==> sub_tex_files/data_construction.tex <==
In this study, we utilized a collection of EHRs sourced from an anonymized institution. The identification of medical jargon within these EHRs was performed using the MedJEx, as detailed in \citet{kwon2022medjex}. Domain experts provided lay definitions for these jargon terms, forming the dataset known as README. For training our models, it was necessary to define these jargon terms in a general yet scientifically accurate manner. To this end, we employed UMLS to generate general definitions. 
UMLS is a set of files and software that brings together many health and biomedical vocabularies and standards to enable interoperability between computer systems. We used the Scispacy library to access UMLS definitions of jargon terms. 
we used the \textit{en\_core\_sci\_lg} model to obtain the data. we tried other models in Scispacy but found all the other models to produce the same result as the \textit{en\_core\_sci\_lg} model~\footnote{\url{https://github.com/allenai/scispacy}}.

Given the complexity of medical terminology, it's noteworthy that some terms in UMLS are associated with multiple definitions. This reflects the reality that the meaning and application of a medical term can vary based on its contextual use. To accurately select the most appropriate general definition for each context, we utilized the SentenceBERT similarity score, as proposed by \citet{reimers2019sentence}, to identify the most fitting definition.    

Jargon terms in our dataset varied in length and composition, with not all words necessarily having corresponding UMLS definitions. This variability necessitated the development of distinct approaches for different scenarios:

\begin{enumerate}
[topsep=0.5pt,itemsep=0.2ex,partopsep=0.2ex,parsep=.20ex]
    \item \textbf{Single-word Terms:} In cases where the jargon term comprised a single word, we either found a UMLS definition or none. Data points lacking a UMLS definition in this category were excluded.
    \item \textbf{Two-word Terms:} For jargon terms composed of two words (word1 and word2), we considered several subcases:
    \begin{enumerate}
        \item Only word1 has a UMLS definition.
        \item Only word2 has a UMLS definition.
        \item Both word1 and word2 have UMLS definitions.
        \item The phrase ``word1 word2'' has a collective UMLS definition.
    \end{enumerate}
    % \item \textbf{Terms with More than Two Words:} This category included terms with varying combinations of words having UMLS definitions. We considered all permutations of word sets within this category.
    \item \textbf{Terms with More than Two Words:} Similar to the case with two words, we can have cases where few words have UMLS definitions in the jargon term and few do not. 
\end{enumerate}

\begin{figure}%[H]
    \centering
    \includegraphics[width=0.75\linewidth]{figs/general_definition.png}
    \caption{General definitions of two jargon examples.}
    \label{fig:general_definition}
    \vspace*{-5mm}
\end{figure}


Our solution to address these scenarios involved a unified approach, given the impracticality of tackling each case individually. As illustrated in Figure~\ref{fig:general_definition}, we extracted the UMLS definitions for all phrases within a jargon term. This process yielded a list of strings, providing a comprehensive general definition for each term. There might not be a UMLS definition for all the words in the jargon term. In that case, we are concatenating the word directly. Subsequently, we applied LLMs for the necessary data-cleaning steps.

The initial README dataset has a lot of unusable data. There are many reasons why a data point might not be useful. The main reasons are (i) the lay definition provided by the annotator is not correct or missing. (ii) The jargon term is missing. (iii)The general definition obtained from UMLS is too scientific or not relevant to the jargon term.
Using this data for training would be bad for the training as these data points will make the model worse. So these data points are not considered. This preliminary cleaning brings out data from 350K to 308K.


==> sub_tex_files/data_selection.tex <==
We adopted four distinct sampling strategies to integrate the AI-synthetic README-v5 data with the expert-annotated README-v2 dataset:

\begin{itemize}
[leftmargin=.2in,topsep=2pt]
\setlength\itemsep{0.01em}
\vspace{-0.2em}
    \item \textbf{RANDOM:} This approach randomly selected N entries from the README-v5 dataset. This is the baseline for our subsequent three heuristic methods.
    \item \textbf{SYNTAX:} For the syntax-based sampling approach, the ROUGE\_L metrics F1 score in Section~\ref{Sec:evaluation} was used as a key evaluative tool. ROUGE\_L focuses on the longest common subsequence, which measures the longest string of words that occurs in both the predicted and reference texts. 
    By using this metric, we could rank the synthetic definitions according to their syntactic closeness to the human-written definitions, which helped us select samples that would potentially be more understandable and natural-sounding.
    \item \textbf{SEMANTIC:} For semantic-based sampling, we utilized the \textit{all-MiniLM-L6-v2} model from the SentenceTransformers framework~\footnote{\url{https://github.com/UKPLab/sentence-transformers}}. 
    Renowned for its text semantic analysis efficiency, this model enabled us to measure the semantic similarity between lay definitions in README-v2 and README-v5 datasets. We ranked synthetic data based on these scores, considering higher scores as indicative of greater semantic closeness to expert annotations.
    \item \textbf{MODEL:} In model-based sampling, 
    we used models initially trained on the README-v2 dataset to generate definitions for the README-v5 dataset. This tested the model's capacity to transfer learnings from expert data to synthetic data. We employed the ROUGE\_L F1 score to evaluate the alignment between model-generated and actual README-v5 lay definitions. 
    This technique aids in mitigating training challenges associated with data heterogeneity and enriches the dataset with examples that enhance the model's convergence towards the desired distribution (e.g., expert-annotated lay definitions).
\end{itemize}


==> sub_tex_files/experimental_setting.tex <==
We use the following symbols:
\begin{enumerate}[topsep=0.5pt,itemsep=0.2ex,partopsep=0.2ex,parsep=.20ex]
    \item jargon2lay(J2L): Directly generates a lay definition for a given jargon term.
    \item jargon+context2lay(J+C2L): Generates a lay definition for a given jargon term based on the context information from clinical documents.
    \item jargon+gen2lay(J+G2L): Generates a lay definition for a given jargon term based on the general definition provided by UMLS.
    \item jargon+context+gen2lay(J+C+G2L): Generates a lay definition for a given jargon term based on both the context information from clinical documents and the general definition provided by UMLS.
\end{enumerate}

We use the following base models: GPT-2 \footnote{\url{https://huggingface.co/gpt2}} \cite{radford2019language}, DistilGPT2 \footnote{\url{https://huggingface.co/distilgpt2}}, BioGPT \footnote{\url{https://huggingface.co/microsoft/biogpt}} \cite{10.1093/bib/bbac409}, and Llama2 \footnote{\url{https://huggingface.co/meta-llama/Llama-2-7b-chat-hf}} \cite{touvron2023llama} in our experiments.
We trained the base models on the different README dataset variants with Supervised Fine-tuning for 100000 steps (batch size 8) \footnote{We did all the experiments with 1 NVIDIA Tesla RTX 8000 GPU - 40 GB memory, with Adam optimizer -- betas=(0.9,0.999), epsilon=1e-08, learning rate=5e-04.}.
In all our evaluations, we used a beam size of 4, no-repeat-ngram-size=2, and minimum length and maximum length of sentences were set as (10, 100). We used five different random seeds to sample training data for all our experiments, and the scores reported in the tables are the average of these random seeds.


\begin{table}[ht]
\scalebox{0.7}{
\setlength{\tabcolsep}{3.9pt}
\renewcommand{\arraystretch}{1.05}
\vspace*{-3mm}
\centering
\begin{footnotesize}
\begin{tabularx}{0.65\textwidth}{X} 

\hline
In this task, we ask for your expertise in generating the corresponding lay definition from the medical jargon. Mainly, we provide the target medical jargon term. We need you to generate a lay definition for this jargon term.
\newline
\newline
Example:
\newline
jargon term: [TERM]
\newline
lay definition: [DEFINITION]
\newline
\newline
jargon term: [TERM]
\newline
lay definition:
\\
\hline
\end{tabularx}
\end{footnotesize}
}
\vspace*{-3mm}
\caption{One shot prompt for experiment set-1.}
\label{one_shot_prompt}
\vspace*{-3mm}
\end{table}

Our experiments were divided into five distinct parts.
In \textbf{Set-1}, we aimed to evaluate the performance gap on the jargon2lay task between open-source base models and GPT models. We do one-shot prompting for Llama2, GPT-3.5-turbo, and GPT-4 with prompts in Table~\ref{one_shot_prompt}. 
\textbf{Set-2} explored the varying data quality across different versions within our EAE pipeline, where we fine-tuned the GPT-2 model on the jargon+gen2lay task.
\textbf{Set-3} focused on evaluating the effects of various data selection strategies on data augmentation outcomes. 
To do this, we ranked AI-generated data (v5) using different methods in Section \ref{Sec:data-selection}, selecting either the top N entries with the highest scores (e.g., `SEMANTIC' in Table~\ref{table:data_selection_results}) or the bottom N entries with the lowest scores (e.g., `SEMANTIC\_r'). 
These selections were then evenly combined with expert-annotated data (v2) at a one-to-one ratio. 
Following this, we fine-tuned the GPT-2 model using these diverse, mixed datasets to determine the impact of each selection method on model performance.
In \textbf{Set-4}, we investigated the effects of incorporating different types of information (medical documentation context and UMLS-retrieved general definition) into the model inputs. 
In \textbf{Set-5}, we fine-tuned models of varying sizes (ranging from DistilGPT2-88M to Llama2-7B) and compared the outcomes with GPT-3.5-turbo.
The next section (Section~\ref{Sec:human_eval}) further validates the findings obtained through this section's automatic evaluation with a comprehensive human evaluation approach.


==> sub_tex_files/human_eval.tex <==
\subsection{Human Evaluation settings}
Our human evaluation was conducted by 5 human evaluators~\footnote{All of whom hold bachelor's degrees}. 
We randomly selected 50 pairs of (jargon, lay definitions) from the test dataset for this human evaluation. 
The task for evaluators was to reference the expert definitions and choose a binary preference among the following four groups of definitions: 
1) DistilGPT2-J2L vs. GPT-3.5-turbo, 
2) DistilGPT2-J+C+G2L vs. GPT-3.5-turbo,
3) LLAMA2-J2L vs. GPT-3.5-turbo, 
4) LLAMA2-J+C+G2L vs. GPT-3.5-turbo. 


\subsection{Human Evaluation Results}
\begin{figure}%[H]
    % \begin{center}
    \vspace{-2mm}
    \centering
    \includegraphics[width=0.7\linewidth]{figs/human_eval.png}
    % \end{center}
    %\setlength{\belowcaptionskip}{-8pt}
    %\setlength{\belowcaptionskip}{-10pt}
    % \setlength{\belowcaptionskip}{-10pt}
    % \vspace*{-3mm}
    \vspace{-4mm}
    \caption{Human evaluation results (win rate).}
    \label{fig:human_eval_results}
    \vspace{-4mm}
\end{figure}


As shown in Figure~\ref{fig:human_eval_results}, although the result of adding context and general definition (DistilGPT2-J+C+G2L) is better than DistilGPT2-J2L, the win rate of the two DistilGPT2 models' output is still significantly behind the result of GPT-3.5-turbo. For LLAMA-2, generating lay definitions directly from jargon is still not as good as GPT-3.5-turbo, but adding context and general definitions is of great help. Human evaluators prefer LLAMA2-J+C+G2L more than GPT-3.5-turbo.
There are some inconsistencies between the results of human evaluation and automatic evaluation. We further interviewed two medical students~\footnote{Both have hospital internship experience} and concluded the following conclusions to help future improvements:
1. While all our in-house systems perform satisfactorily, GPT-3.5-turbo stands out for its flexibility and user-friendliness. Particularly, it excels in elaborating complex medical terms, offering detailed explanations and practical examples for better comprehension.
2. Recent advancements~\cite{cai2023paniniqa, zhang2023ehrtutor} reveal ChatGPT's role in enhancing patient education through interactive formats like NoteAid-interactive~\cite{NoteAid-interactive}. 
It enables patients to actively ask questions and seek clarifications, while the AI tailors responses to aid their understanding. This interactive approach, absent in traditional dictionary-style definitions like our README dataset, calls for next-step model distillation work or further refinement in aligning the in-house system's outputs with patient preferences. 
Additionally, the development of automatic metrics aligning closely with human evaluation is another critical next step.


==> sub_tex_files/introduction.tex <==
The advancement in healthcare transcends medical breakthroughs, encompassing an increased emphasis on patient involvement in self-care~\cite{HomeHealthCare, nurseNavigators, baldry1986giving, schillinger2009effects}. The criticality of effective patient education is underscored in an era marked by the emergence of new treatments that demand patient comprehension and cooperation. 
Access to Electronic Health Records (EHR) has become an integral part of this educational paradigm, with initiatives like PCASSO~\cite{GivingPatientsAccess} and NoteAid~\cite{chen2018natural,kwon2022medjex} leading the way in empowering patients and enhancing healthcare outcomes.
These efforts demonstrate a shift towards patient-centric healthcare, where informed patients play an active role in their treatment processes.



Despite advancements in electronic medical record management, one significant barrier persists in the form of medical jargon in EHRs, impeding patient understanding and self-care~\cite{kwon2022medjex}. 
As shown in Figure~\ref{fig:noteaid}, tools like NoteAid, which employs Natural Language Processing (NLP) to demystify complex medical terms, have been instrumental in bridging the communication gap between healthcare professionals and patients~\cite{lalor2018comprehenotes, lalor2021evaluating, lalor2023evaluating}. 
However, existing resources
%scope of layperson-accessible explanations in existing resources 
like the Consumer Health Vocabulary (CHV)~\cite{zeng2006exploring, he2017enriching, ibrahim2020enriching} are limited in scale, 
%used by NoteAid 
posing a challenge to NoteAid. For instance, only a fraction (about 4\%) of the medical terms in NoteAid have been annotated with lay definitions,
%in NoteAid have comprehensible explanations, 
highlighting the need for a more 
%comprehensive 
scalable solution to address this knowledge gap effectively.




Addressing this issue requires shifting our focus to online health education materials such as Unified Medical Language System (UMLS) ~\cite{bodenreider2004unified}, MedlinePlus~\cite{patrias2007citing}, Wikipedia, and Google. 
However, as indicated in Figure \ref{fig:noteaid}, these resources often present information that is too difficult for the average patient to understand. For example, these resources' average readability measured by the Flesch Kincaid Grade Level was post-secondary or higher education, while the average readability of a US adult was 7-8th grade level~\cite{doak1996teaching, doak1998improving, eltorai2014readability}.
To bridge this gap, we have engaged a team of medical experts to meticulously curate lay definitions for jargon terms found in NoteAid, targeting a comprehension level suitable for individuals with a 7th to 8th-grade education.
Each term within the NoteAid dataset has been redefined across various contexts, ensuring their applicability in diverse clinical scenarios. 
This effort led to the creation of the REsource of lAy Definitions for MEdical jargon (README) dataset, an expansive resource containing lay definitions for over 20,000 medical terms.
In total, the README dataset comprises an impressive 300,000 data points, each consisting of a clinical note context, a medical jargon term, and its corresponding lay definition, thereby significantly enhancing the accessibility and comprehensibility of medical information for patients.


\begin{figure}[H]
    \centering
    \vspace*{-4mm}
    \includegraphics[width=0.8\linewidth]{figs/noteaid_and_definition.png}
    \vspace*{-5mm}
    \caption{The NoteAid pipeline comprises an NLP component and a resource of medical jargon and the corresponding lay definitions. We list definitions for the term "EGD" across various online sources registered Flesch-Kincaid Grade Level (FKGL) above 13, suggesting they are comprehensible mainly to individuals with post-secondary education.}
    \label{fig:noteaid}
    \vspace{-4mm}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=0.7\linewidth]{figs/human-ai-loop.png}
    \vspace*{-5mm}
    \caption{Our Human-AI-in-the-loop Data-Centric NLP pipeline, comprising 
    the Examiner-Augmenter-Examiner (EAE) framework and different data selection methods.
    %Following the Human-AI-in-the-loop paradigm, 
    EAE shows how humans (physicians) and AI (LLM, e.g. ChatGPT) cooperate to make a high-quality README dataset.
    We collect general definitions for every jargon term from external knowledge resources such as UMLS. ``R’' is ``README’'. ``v1’' is ``version-1’'. ``instruction’' and ``demo’' (examples for in-context learning) are combined into the prompt for LLM.
    In the pipeline, the human duties at different stages are annotator (labeling the initial dataset) and instructor (providing suitable prompts to guide AI at every stage). 
    The AI duties at different stages are examiner (filter high-quality data) and augmenter (improve the quality of low-quality data).
    We then deploy 4 different data selection strategies to combine high-quality expert-annotated data R-v2 and high-quality AI-synthetic data R-v5 and train the in-house system.
    }
    \label{fig:human-ai-loop}
    \vspace*{-5mm}
\end{figure*}

Yet, the critical aspect of generating lay definitions remains largely unexplored.
As patients gain more access to their EHRs, the demand for lay definition resources is escalating, inevitably destined to surpass the capacity of current expert-annotated resources, regardless of efforts to expand them. 
In addition, the dynamic nature of "jargon" based on individual and context makes pre-annotated expert resources less adaptable to real-life scenarios. 
The model-driven automatic generation of lay definitions from medical jargon emerges as a viable solution. 
Recent research highlighted ChatGPT's potential in its integration with the field of medicine~\cite{brown2020language,openai2023gpt4,yang2023performance}, including generating human-readable definitions for biomedical terms~\cite{remy2023automatic}. Nonetheless, our evaluations of open-source models (refer to Figure~\ref{fig:one_shot_performance}) indicate notable differences in their performance compared to ChatGPT, particularly in terms of medical knowledge~\cite{sung2021can, yao2022extracting, yao2023context}. 


To bridge this gap, we aim to train an in-house system using open-source models for automatic lay definition generation to provide reliable lay definitions for jargon in patient education tools like NoteAid. 
Inspired by research on Retrieval-Augmented Generation (RAG) ~\cite{lewis2020retrieval,asai2023self}, we aim to overcome the limitations of open-source base models in medical knowledge. 
We are positioning automatic lay definition generation as a form of text simplification, where language models are prompted to generate context-aware, jargon-specific, and layperson-friendly definitions based on standard definitions retrieved from external knowledge resources. 
Specifically, in this work, we use the UMLS to retrieve standard definitions of jargon terms and construct a dataset upon the README that includes context, jargon terms, standard definitions, and lay definitions.



Subsequently, we designed the data-centric pipeline Examiner-Augmenter-Examiner (EAE) to enhance the data quality within the README dataset, as seen in Figure \ref{fig:human-ai-loop}. 
Specifically, following a human-in-the-loop paradigm~\cite{monarch2021human}, we employed human experts to guide AI in both examiner and augmenter stages, where the former selects high-quality training data (originating from either manual annotation or AI synthesis), and the latter generates potentially high-quality synthesized data to increase data points.
Finally, we employed the AI-synthesized dataset to augment the expert-annotated dataset, aiming to explore the effectiveness of AI-generated data in training, especially in scenarios with limited expert data. 
We implemented a range of heuristic data selection strategies to integrate AI synthetic data, allowing us to incorporate suitable data points into our training process.



\noindent{\textbf{In summary, our contributions are as follows:}}
\begin{itemize}   
[leftmargin=.2in,topsep=0.1pt]
\setlength\itemsep{-0.2em}
\vspace{-0.2em}
    \item Introduced a new task of automatically generating lay definitions for medical jargon.
    We created a substantial expert-annotated dataset containing 300,000 data points, serving as a detailed dictionary and a benchmark for this novel task. 
    We leveraged a Retrieval-Augmented Generation (RAG) method, which aims to reduce hallucinations and improve the quality of model outputs. 
    Our work aims to enhance patient education by improving patients' comprehension of medical documentation.

    \item Developed a robust, data-centric pipeline that effectively integrates data filtering, augmentation, and the selection of synthetic data. This approach enhances the quality of README datasets, merging the strengths of AI with human expertise to achieve optimal results.

    \item Our extensive automatic and human evaluations reveal that when trained with high-quality data, open-source, mobile-friendly small models can achieve or even exceed the performance of cutting-edge closed-source large language models, such as ChatGPT.

\end{itemize}

==> sub_tex_files/limitation_ethical.tex <==
This study provides valuable insights, but experimental results evaluated in humans demonstrate limitations of the current work and some future directions. First, better automatic evaluation metrics need to be explored to be closer to human evaluation results. Secondly, in this paper, we have only explored some heuristic data selection methods, and we need to explore more sophisticated methods in the future. In addition, the next step of the in-house system is to collect patient preferences for human alignment, which can help us generate a more user-friendly or customized lay definition. Also, we can use ChatGPT or LLAMA2-J-C-G2L to serve as the teacher and use DistilGPT2-based systems to serve as the students, performing distillation to improve the performance of the small models post current supervisor-fine-tuning on README. Finally, more interactive ways need to be considered in the future to make the in-house system more user-friendly and patient-centric.



Consider Privacy Implications, LLMs (especially third-party APIs like ChatGPT) may raise privacy concerns when conducting patient education, which may violate HIPAA regulations. In this study, we manually annotated lay definitions on publicly available MedJEx jargon terms and obtained general definitions from accessible UMLS. We also make AI-synthetic data to help training since synthetic data generation is an active field in the clinical domain especially to overcome privacy concerns~\cite{pereira2022secure,shafquat2022source,mishra2023synthetic}.
The trained in-house system can be deployed on the patient's mobile to avoid patient data leaving the local area, which can better protect the patient's privacy and security. Consider Biases, LLMs trained on large amounts of text data may inadvertently capture and reproduce biases present in the data. Therefore, an in-house system trained on our data (whether expert annotation or AI synthetic) may perpetuate incorrect information or provide inaccurate answers. Finally, although we used UMLS-based RAG to reduce hallucinations, LLMs may still generate factual errors when conducting patient education.

==> sub_tex_files/problem_statement.tex <==
Consider a dataset \(D = \{X, Y, Z_{+}\}\) comprising \(t\) EHRs, where \(X = \{x^1, x^2, \ldots, x^t\}\) represents the contexts of these EHRs, \(Y = \{y^1, y^2, \ldots, y^t\}\) denotes the corresponding jargon terms, and \(Z_{+} = \{z_{+}^1, z_{+}^2, \ldots, z_{+}^t\}\) are the ground truth expert lay definitions. Each EHR context \(x^i\) is a sequence of \(n\) tokens, expressed as \(x^i = \{x_1^{i}, x_2^{i}, \ldots, x_n^{i}\}\), and each lay definition \(z_{+}^i\) consists of \(m\) tokens, given by \(z_{+}^i = \{z_{+,1}^{i}, z_{+,2}^{i}, \ldots, z_{+,m}^{i}\}\). 
The README lay definition generation task \(T\) aims to train a reference model \(M_{ref}\) such that \(M_{ref}(z_{+}^i \mid x^i, y^i)\) is optimized. The standard approach for fine-tuning \(M_{ref}\) on \(T\) involves using the cross-entropy loss \(\ell_{ce}(z_{+}^i, M_{ref}(x^i, y^i))\) over the dataset \(D\).
To enhance the training of \(M_{ref}\), we introduce an additional set of general definitions \(Z_{-} = \{z_{-}^1, z_{-}^2, \ldots, z_{-}^t\}\), where each \(z_{-}^i\) corresponds to the general definition of the jargon term \(y^i\), generated using openly available data sources (UMLS) or GPT-3.5-turbo. Our proposed EAE pipeline is designed to acquire high-quality general definition data \(Z_{-}\), culminating in the augmented dataset \(D_{simp} = \{X, Y, Z_{+}, Z_{-}\}\).
The README lay definition generation task T is then formalized as a text simplification task, where \(M_{ref}\) is trained to produce \(Z_{+}\) based on \(X, Y,\) and \(Z_{-}\). This process utilizes a selected subset \(D_{SEL} \subseteq D_{simp}\), chosen according to one of the selection criteria: RANDOM, SYNTAX, SEMANTIC, or MODEL.


==> sub_tex_files/related_work.tex <==
\noindent\textbf{Data-Centric AI}
In the Data-centric AI framework, the README meticulously navigates through the collection, labeling, preparation, reduction, and augmentation phases~\cite{zha2023data, ng2021data}. 
README begins with data collection and labeling (\ref{Sec:data_construction}), harnessing domain expertise to curate a dataset that is both expansive and representative~\cite{whang2023data}.
During the preparation phase (\ref{Sec:data-centric}), raw data undergoes rigorous cleaning and transformation, readying it for effective model training~\cite{krishnan2019alphaclean}.
README also adeptly applies data augmentation techniques (\ref{Sec:data-centric}) to enrich the dataset with verified quality AI-synthetic data~\cite{chlap2021review}.
Finally, through data reduction (\ref{Sec:data-selection}), README selects more suitable instances from AI-synthetic data for data integration with expert-annotated data~\cite{whang2023data}.
Collectively, these stages underscore README's comprehensive application of Data-centric AI in the healthcare domain.

% Data-centric AI refers to a framework to develop, iterate, and maintain data
% for AI systems [269]. Data-centric AI involves the tasks and methods for building effective
% training data, designing proper inference data, and maintaining the data.
% Collection Labeling Preparation Reduction Augmentation

% Data Collection
% Data collection is the process of gathering and acquiring data from various sources, which fundamentally determines data quality and quantity. This process heavily relies on domain knowledge.
% With the increasing availability of data, there has been a surge in the development of efficient
% strategies to leverage existing datasets. In the following, we discuss the role of domain knowledge,
% an overview of more efficient data collection strategies, and challenges.

% Data Labeling
% Data labeling is the process of assigning one or more descriptive tags or labels to a dataset, enabling
% algorithms to learn from and make predictions on the labeled data. Traditionally, this is a timeconsuming and resource-intensive manual process, particularly for large datasets. Recently, more
% efficient labeling methods have been proposed to reduce human efforts. In what follows, we discuss
% the need for data labeling, efficient labeling strategies, and challenges.

% Data Preparation
% Data preparation involves cleaning and transforming raw data into a format that is appropriate for
% model training. Conventionally, this process often necessitates a considerable amount of engineering
% work with laborious trial and error. To automate this process, state-of-the-art approaches often
% adopt search algorithms to discover the most effective strategies. In this subsection, we introduce
% the need, representative methods, and challenges for data preparation

%  Data Reduction - Methods for Reducing Sample Size. 
% The reduction of samples is typically achieved with
% instance selection, which selects a representative subset of data samples that retain the original
% properties of the dataset. The existing studies can be divided into wrapper and filter methods.
% The former selects instances based on scoring functions. For example, a common strategy is to
% select border instances since they can often shape the decision boundary [193]. Wrapper methods,
% in contrast, select instances based on model performance [225], which considers the interaction
% effect with the model. Instance selection techniques can also alleviate data imbalance issues by
% undersampling the majority class, e.g., with random undersampling [186]. More recent work adopts
% reinforcement learning to learn the best undersampling strategies [148]. Overall, instance selection
% is a simple yet effective way to reduce data sizes or balance data distributions

% Data Augmentation
% Data augmentation is a technique to increase the size and diversity of data by artificially creating
% variations of the existing data, which can often improve the model performance. It is worth noting
% that even though data augmentation and data reduction seem to have contradictory objectives, they
% can be used in conjunction with each other. While data reduction focuses on eliminating redundant
% information, data augmentation aims to enhance data diversity. We will delve into the need for
% data augmentation, various representative methods, and the associated challenges.



\noindent\textbf{Patient Education}
Patient education plays a crucial role in the success of therapy \citep{bastable2016essentials, golper2001patient}. Elevating the level of patient education has consistently been an important component within the healthcare system \citep{mccarthy2013understanding}. 
By providing clear and easily understandable medical information, patient education not only enhances patients' awareness of their own health conditions but also encourages them to actively participate in medical decision-making and self-management\citep{GRUMAN2010350, coulter2012patient}.
NoteAid \citep{chen2018natural} transforms complex medical terms in EHR notes into understandable language, integrating advanced features like MedJEx \citep{kwon2022medjex} to enhance patient comprehension.
Efforts to demystify clinical language have also been made in the works of ~\citet{petrova2014learning,petrova2015formalizing}, while \citet{remy2023automatic} successfully employed ChatGPT for generating accurate medical definitions.



% \section{Related Work (WIP)}
% \paragraph{Definition Generation}

% % [1] S Kwon et al., “Vision Meets Definitions: Unsupervised Visual Word Sense Disambiguation Incorporating Gloss Information”, Under review (will publish Arxiv after May 3rd)

% % [2] Malkin et al., “GPT Perdetry Test: Generating new meanings for new words”, ACL 2021

% % [3] Li et al., Explicit Semantic Decomposition for Definition Generation, ACL 2020

% % [4] Gadetsky et al., “Conditional generators of words definitions.” ACL 2018

% % [5] Noraset et al., Definition modeling: Learn- ing to define word embeddings in natural language, AAAI 2017

% % [6] Background Knowledge Grounding for Readable, Relevant, and Factual Biomedical LaySummaries

% % The task of definition generation was introduced in natural language processing by Noraset et al. (2017) with the aim of creating a definition for a given word. To accomplish this task, Noraset et al. suggest using recurrent neural network-based language models (RNNLMs) with definitions gathered from WordNet and GCIDE. Other researchers have proposed various methods to improve definition generation, such as using context and the soft-attention mechanism to handle polysemous words (Gadetsky et al., 2018), conducting semantic decomposition of word meanings and using discrete latent variables (Li et al., 2020), and generating definitions of neologisms with a large pretrained language model such as GPT-3 (Malkin et al., 2021, Kwon et al., 2023). Especially, Kwon et al. (2023) not only demonstrated that GPT-3 c but also showed that the generated definitions can adopt to a downstream task, visual word-send disambiguation.
% \citet{noraset2017definition} suggested the definition generation via recurrent network-based language models (RNNLMs) to generate definitions for specific words on data with WordNet and GNU Collaborative International Dictionary of English
% (GCIDE).
% \citet{gadetsky2018conditional} suggested leveraging context and soft-attention mechanisms to manage polysemous words, while \citet{li2020explicit} recommended semantic decomposition of word meanings and using discrete latent variables. Recent studies suggested to utilize large language models such as GPT-3 for the definition generation \citep{malkin2021gpt, kwon-etal-2023-vision}. Notably, \citet{kwon-etal-2023-vision} not only showcased the capabilities of GPT-3 but also demonstrated how the produced definitions could be adapted for a subsequent task; visual word-sense disambiguation \citep{raganato2023semeval}.

% % Bridging the Literacy Gap for Surgical Consents: An AI-Human Expert Collaborative Approach (using GPT4)


% \paragraph{The impact of training data noise} is less studied. The most common proposal is to identify low-quality samples–with entailment \cite{matsumaru2020improving, goyal2021annotating} or entity overlap (Nan et al., 2021a; Narayan et al., 2021)–and drop them. These filtering methods tend to improve faithfulness yet can degrade informativeness. Kang and Hashimoto (2020) address the data hunger issue by first training on all samples before implementing Loss Truncation–ignoring high log loss datapoints. This is effective on a relatively clean Gigaword corpus yet untested on noisier corpora in which hallucination behavior from the unfiltered data may be difficult to unlearn. Filtering can be “insufficient to train a competitive model” when high-quality data is limited (Filippova, 2020). \citet{adams2022learning} consider a noisier, lower resource setting (clinical summarization) and propose a new approach: to revise–not remove–noisy reference content.

% % https://arxiv.org/abs/2308.16361.pdf

% \paragraph{Data Augmentation} is a common technique in NLP for counteracting the limited data available with few-shot learning (Feng et al., 2021; Chen and Yin, 2022). Flavors of data augmentation include surface form alteration (Wei and Zou, 2019), latent perturbation (Sennrich et al., 2016; Fabius et al., 2015) or auxiliary supervision (Chen and Yu, 2021). Our method can be considered a form of text generation with transformers (Kumar et al., 2020; Ng et al., 2020), which lately rely on increasingly larger language models (Yoo et al., 2021; Wang et al., 2021a,b). Whereas these methods paraphrase or pseudo-label a seed utterance, MSP instead conditions on a label to control the generation of text.

==> sub_tex_files/results.tex <==

We start with our experiments with some base models' performance on the README jargon2lay dataset with In \textbf{Set-1}.
In Section \ref{method:soft_hard_correlation}, we noted a high level of agreement between human evaluators and definitions generated by GPT-3.5-turbo. 
This aligns with the findings of recent work by \citet{remy2023automatic}, which underlines GPT-3.5-turbo's efficacy in crafting human-readable explanations for biomedical concepts. 
Consequently, GPT-3.5-turbo serves as a strong baseline for quality in README lay definition generation, indicative of a standard that meets human satisfaction. 
Despite this, our assessments of Llama2, depicted in Figure~\ref{fig:one_shot_performance}, show a notable gap in performance. 
% Llama2 and more small LMs (e.g., DistilGPT2, GPT2, BioGPT) fall short of the GPT-3.5-turbo benchmark. 
This disparity underscores the urgent need to upgrade the performance of Llama2 and other open-source models (e.g., DistilGPT2, GPT2, BioGPT) to align with the high-quality output of GPT-3.5-turbo.
Finally, We also observed that GPT-3.5-turbo and GPT4 performed equally well in this task.
Next, we discuss how different modules of our data-centric pipeline improve the performance of the fine-tuned models in several subsections.

\begin{figure}[H]
    % \begin{center}
    \centering
    \includegraphics[width=0.7\linewidth]{figs/one_shot_comparision.png}
    % \end{center}
    %\setlength{\belowcaptionskip}{-8pt}
    %\setlength{\belowcaptionskip}{-10pt}
    % \setlength{\belowcaptionskip}{-10pt}
    % \vspace*{-3mm}
    \vspace{-4mm}
    \caption{One-shot performances on jargon2lay.}
    \label{fig:one_shot_performance}
    \vspace{-4mm}
\end{figure}


\subsubsection{Effectiveness of EAE pipeline}


\begin{table}[H]
\vspace{-4mm}
\centering
\scalebox{0.64}{
\begin{tabular}{c|ccccc|c}
\hline


\hline
J+G2L  & \small{ROUGE1} &  \small{ROUGE2} & \small{ROUGEL} & \small{METEOR} & \small{UMLS-F1} & \small{Rank}
\\

\hline

v1 & 23.94 & 8.95 & 22.79 & 17.75 & 12.83 & 2
\\
v2 & 26.99 & 10.76 & 25.57 & 21.19 & 16.88 & 4
\\
v3 & 22.25 & 7.46 & 21.09 & 17.18 & 11.72 & 5
\\
v5 & 25.71 & 9.75 & 24.41 & 20.23 & 16.01 & 3
\\
v2+v5 & 29.82 & 13.14 & 28.47 & 24.42 & 20.09 & 1
\\

\hline

\end{tabular}
}
\vspace{-4mm}
\caption{Various README versions data performance.} 
\label{table:EAE_results}
\vspace{-3mm}
\end{table}


In \textbf{Set-2}, we focus on the efficacy of different data versions when finetuning with the GPT-2 model. 
The results, as reflected in Table~\ref{table:EAE_results}, indicate that high-quality expert data (v2) demonstrates clear superiority over unexamined expert data (v1), emphasizing the crucial role of ECE-examiner in enhancing data quality. 
Furthermore, high-quality synthetic data (v5) outperforms the unexamined expert data (v1), underscoring the significant value of data augmentation in the ECE pipeline. 
Notably, the combination of v2 and v5 shows improved performance over v2 alone, suggesting that including synthetic data is beneficial.
This composite approach of v2+v5 leading the rank underscores the efficacy of our EAE Human-AI team.



% gpt2, jargon+gen2lay, unexamined expert data (v1), high-quality expert data (v2), low-quality expert data (v3), high-quality synthetic data (v5). 
% The superiority of version 2 (v2) over version 1 (v1) highlights the significance of the examiner's role in the process. Additionally, the fact that version 5 (v5) outperforms v1 underscores the importance of data augmentation. The improved performance of v2+v5 compared to v2 alone suggests that v5 is necessary when v2 alone is insufficient. Overall, this indicates that our EAE pipeline is essential for the process.


\subsubsection{Expert and Synthetic Data Integration}

\begin{table}[H]
\vspace{-4mm}
\centering
\scalebox{0.62}{
\begin{tabular}{c|cccc}
\hline


\hline
\small{ROUGE1} &  \small{J2L} & \small{J+C2L} & \small{J+G2L} & \small{J+C+G2L}
\\

\hline
RANDOM & 19.03 & 19.65 & 26.21 & 26.97
\\
SYNTAX(R) & 19.82(\textcolor{red}{-2.28}) & 20.65(\textcolor{red}{-2.78}) & 27.56(\textcolor{red}{-8.36}) & 28.33(\textcolor{red}{-8.84})
\\
SEMANTIC(R) & 19.74(-1.11) & 19.94(-1.39) & 26.42(-0.92) & 27.19(-1.96)
\\
MODEL(R) & 20.18(-0.8) & 20.46(-1.88) & 27.9(-2.37) & 28.65(-4.22) 
\\
\hline

\small{UMLS-f} &  \small{J2L} & \small{J+C2L} & \small{J+G2L} & \small{J+C+G2L}
\\

\hline
RANDOM & 8.05 & 9.09 & 15.78 & 16.72
\\
SYNTAX(R) & 8.53(-0.11) & 9.99(\textcolor{red}{-1.00}) & 17.76(\textcolor{red}{-5.11}) & 17.42(\textcolor{red}{-5.54})
\\
SEMANTIC(R) & 8.98(-0.38) & 9.07(-0.69) & 15.93(-0.02) & 16.74(-0.93)
\\
MODEL(R) & 9.18(\textcolor{red}{-0.63}) & 9.4(-0.78) & 18.34(-2.5) & 18.45(-2.55)
\\

\hline

\end{tabular}
}
\vspace{-4mm}
\caption{Different data selection methods performance.} 
\label{table:data_selection_results}
\vspace{-3mm}
\end{table}

In \textbf{Set-3}, we explored the effects of various data selection strategies on data augmentation outcomes. 
We found that, compared to the other two methods, the results of SEMANTIC are closer to RANDOM. 
Also, the SEMANTIC-based ranking remained fairly consistent between SEMANTIC and SEMANTIC\_r.
However, significant differences were observed in SYNTAX and SYNTAX\_r, MODEL and MODEL\_r.
Table~\ref{table:data_selection_results} highlights two main findings: 
firstly, data selection is crucial, as all methods have better performance with higher-ranked data (e.g., SYNTAX, SEMANTIC, MODEL) over lower (e.g., SYNTAX\_r, SEMANTIC\_r, MODEL\_r). 
All three methods, SYNTAX, SEMANTIC, MODEL, have better results than the RANDOM baseline.
Secondly, the effectiveness of a selection algorithm is proportional to the range it creates between the top and last ranking items, with a larger gap indicating a more effective selection process.
This implies that with an equal volume of v5 data, the selection methods prioritize data that maximizes the benefits of augmentation and relegates the least impactful data to the lower echelon.



\subsubsection{Retrieval-augmented Generation}
\begin{table}[H]
\vspace{-4mm}
\centering
\scalebox{0.57}{
\begin{tabular}{c|ccccc}
\hline


\hline
& \small{ROUGE1} &  \small{ROUGE2} & \small{ROUGEL} & \small{METEOR} & \small{UMLS-F1}
\\


& \multicolumn{5}{c}{Without data augmentation (v2)}
\\
\hline

jargon2lay & 19.47 & 6.06 &	18.53 &	14.74 & 8.76
\\
jargon+context2lay & 19.40 & 6.40 & 18.38 & 15.12 & 9.24
\\
jargon+gen2lay & 26.99 & 10.76 & 25.57 & 21.19 & 16.88
\\
jargon+context+gen2lay	 & \textcolor{red}{27.58} & \textcolor{red}{11.31} & \textcolor{red}{26.35} & \textcolor{red}{21.72} & \textcolor{red}{17.12}
\\


\hline
& \multicolumn{5}{c}{With data augmentation (v2+v5 with SYNTAX)}
\\
\hline

jargon2lay & 21.98 & 7.42 &	20.88 & 16.98 & 10.95
\\
jargon+context2lay & 22.13 & 7.90 & 21.04 & 17.54 & 10.71
\\
jargon+gen2lay & 29.82 & 13.14 & 28.47 & 24.42 & 20.09
\\
jargon+context+gen2lay & \textcolor{red}{29.89} & \textcolor{red}{13.48} & \textcolor{red}{28.49} & \textcolor{red}{24.65} & \textcolor{red}{20.27}
\\

\hline

\end{tabular}
}
\vspace{-4mm}
\caption{Efficacy of incorporating medical documentation context and general definition in input data.} 
\label{table:jargon+gen+context}
\vspace{-2mm}
\end{table}


\textbf{Set-4} results underscore the significant improvement in model performance when input data is enriched with UMLS-retrieved general definitions. 
As illustrated in Table~\ref{table:jargon+gen+context}, regardless of whether we utilize only expert-annotated data or data augmentation with AI-synthetic data, including general definitions consistently enhances effectiveness. 
This finding confirms the value of RAG with the general definition in the lay definition generation task. 
Meanwhile, adding context to the input data yields a moderate impact on model performance. 


\subsubsection{Model Performances Against ChatGPT}
\begin{figure}[H]
    \vspace{-4mm}
    % \begin{center}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/lm_results.png}
    % \end{center}
    %\setlength{\belowcaptionskip}{-8pt}
    %\setlength{\belowcaptionskip}{-10pt}
    % \setlength{\belowcaptionskip}{-10pt}
    % \vspace*{-3mm}
    \vspace{-4mm}
    \caption{Comparative performance analysis of DistilGPT2, BioGPT, and LLAMA2 against GPT-3.5-turbo.}
    \label{fig:gpt2_biogpt_llama2_biollama2}
    \vspace{-2mm}
\end{figure}


In \textbf{Set-5}, we observed that LLAMA2-7B's ROUGE-1 and UMLS-F1 metrics surpassed GPT-3.5-turbo in the jargon2lay task post-training. 
For the jargon+gen2lay setting, DistilGPT2-88M demonstrated equivalent results to GPT-3.5-turbo, while BioGPT's performance exceeded it, and LLAMA2-7B significantly outperformed the GPT-3.5-turbo. 
These findings, as depicted in Figure~\ref{fig:gpt2_biogpt_llama2_biollama2}, emphasize the effectiveness of open-source, mobile-adapted smaller models when appropriately fine-tuned with high-quality datasets, offering a promising avenue for deploying lightweight yet powerful NLP tools in mobile healthcare applications to help patient education. 
